Survey of Aspect-based Sentiment Analysis Datasets

Aspect-based sentiment analysis (ABSA) is a natural language processing problem that requires analyzing user-generated reviews to determine: a) The target entity being reviewed, b) The high-level aspect to which it belongs, and c) The sentiment expressed toward the targets and the aspects. Numerous yet scattered corpora for ABSA make it difficult for researchers to identify corpora best suited for a specific ABSA subtask quickly. This study aims to present a database of corpora that can be used to train and assess autonomous ABSA systems. Additionally, we provide an overview of the major corpora for ABSA and its subtasks and highlight several features that researchers should consider when selecting a corpus. Finally, we discuss the advantages and disadvantages of current collection approaches and make recommendations for future corpora creation. This survey examines 65 publicly available ABSA datasets covering over 25 domains, including 45 English and 20 other languages datasets.

==> Sections/tables.tex <==
\begin{table*}[!t]
            \texttt{Restaurant Review  (s)}: The \textbf{\textit{\color{blue}{pasta}}} was \textbf{\textit{\color{red}{very yummy}}} but the \textbf{\textit{\color{blue}{place}}} has some \textbf{\textit{\color{red}{weird smell}}}.\\ \texttt{Aspect Categories:} \{\textit{Food, Ambience, Service, Price, General}\}
            \centering
            \resizebox{\linewidth}{!}{%
            \begin{tabular}{|l|l|lp{2cm}p{2cm}|lll|l|}
            \hline
            \multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Year}}} &
              \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Paper}}} &
              \multicolumn{3}{c|}{\textbf{Info}} &
              \multicolumn{3}{c|}{\textbf{Aspect}} &
              \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Type}}} \\ \cline{3-8}
            \multicolumn{1}{|c|}{} &
              \multicolumn{1}{c|}{} &
              \multicolumn{1}{c|}{\textbf{Common Name}} &
              \multicolumn{1}{c|}{\textbf{Input}} &
              \multicolumn{1}{c|}{\textbf{Expected Output}} &
              \multicolumn{1}{c|}{\textbf{Category}} &
              \multicolumn{1}{c|}{\textbf{Term}} &
              \multicolumn{1}{c|}{\textbf{Target}} &
              \multicolumn{1}{c|}{} \\ \hline
            2004 & \cite{Hu-2004}  & Aspect Term Extraction (ATE)  & \multicolumn{1}{|p{2cm}|}{\texttt{s}} & \multicolumn{1}{p{3cm}|}{\textbf{\textit{\color{blue}{pasta, place}}}} & \multicolumn{1}{l|}{-}              & \multicolumn{1}{l|}{\priority{0}}      & -              & Single \\ \hline
            2014 & \cite{14-dataset} & Aspect Category Detection (ACD)   & \multicolumn{1}{|p{2cm}|}{\texttt{s}} & \multicolumn{1}{p{3cm}|}{\textit{Food, Ambience}} & \multicolumn{1}{l|}{\priority{0}}   & \multicolumn{1}{l|}{-}                 & -              & Single \\ \hline
            2015 & \cite{15-dataset} & Target Detection (TD) & \multicolumn{1}{|p{2cm}|}{\texttt{s}} & \multicolumn{1}{p{3cm}|}{\textbf{\textit{\color{blue}{pasta, place}}}} &  \multicolumn{1}{l|}{-}              & \multicolumn{1}{l|}{-}                 & \priority{0}   & Single \\ \hline
            2004 & \cite{Hu-2004} & Aspect Term Sentiment Analysis (ATSA)  & \multicolumn{1}{|p{2cm}|}{\texttt{s}, (\textbf{\textit{\color{blue}{pasta, place}}})} & \multicolumn{1}{p{2cm}|}{\texttt{positive, negative}} & \multicolumn{1}{l|}{-}              & \multicolumn{1}{l|}{\semipriority{50}} &    -            & Single \\ \hline
            2014 & \cite{14-dataset} & Aspect Category Sentiment Analysis (ACSA) & \multicolumn{1}{|p{2cm}|}{\texttt{s}, (\textit{Food, Ambience})} & \multicolumn{1}{p{2cm}|}{\texttt{positive, negative}} & \multicolumn{1}{l|}{}               & \multicolumn{1}{l|}{\semipriority{50}} &    -            & Single \\ \hline
            2020 & \cite{schmitt-ASD} & Aspect Sentiment Joint Detection (ASD) & \multicolumn{1}{|p{2cm}|}{\texttt{s}} & \multicolumn{1}{p{3cm}|}{(\textit{Food}, \texttt{positive}), (\textit{Ambience}, \texttt{negative})} & \multicolumn{1}{l|}{\priority{50}}  & \multicolumn{1}{l|}{-}                 & -              & Joint  \\ \hline
            2019 & \cite{Li-unified-TSD} & Target Sentiment Joint Detection (TSD) & \multicolumn{1}{|p{2cm}|}{\texttt{s}} & \multicolumn{1}{p{3cm}|}{(\textbf{\textit{\color{blue}{pasta}}}, \texttt{positive}), (\textbf{\textit{\color{blue}{place}}}, \texttt{negative})} & \multicolumn{1}{l|}{-}              & \multicolumn{1}{l|}{-}                 & \priority{50}  & Joint  \\ \hline
            2014 & \cite{14-16-MTNA} & Target Aspect Detection (TAD) & \multicolumn{1}{|p{2cm}|}{\texttt{s}} & \multicolumn{1}{p{3cm}|}{(\textbf{\textit{\color{blue}{pasta}}}, \textit{Food}), (\textbf{\textit{\color{blue}{place}}}, \textit{Ambience})} & \multicolumn{1}{l|}{\priority{0}}   & \multicolumn{1}{l|}{-}                 & \priority{0}   & Joint  \\ \hline
            2020 & \cite{TargetAspectSentimentJD} & Target Aspect Sentiment Joint Detection (TASD) & \multicolumn{1}{|p{2cm}|}{\texttt{s}} & \multicolumn{1}{p{3cm}|}{(\textbf{\textit{\color{blue}{pasta}}}, \textit{Food}, \texttt{positive}), (\textbf{\textit{\color{blue}{place}}}, \textit{Ambience}, \texttt{negative})} & \multicolumn{1}{l|}{\priority{50}}  & \multicolumn{1}{l|}{-}                 & \priority{50}  & Joint  \\ \hline
            2019 & \cite{ASTE-dataset} & Aspect Sentiment Triplet Extraction (ASTE) & \multicolumn{1}{|p{2cm}|}{\texttt{s}} & \multicolumn{1}{p{3cm}|}{(\textbf{\textit{\color{blue}{pasta}}}, \textbf{\textit{\color{red}{very yummy}}}, \texttt{positive}), (\textbf{\textit{\color{blue}{place}}}, \textbf{\textit{\color{red}{weird smell}}}, \texttt{negative})} & \multicolumn{1}{l|}{-}              & \multicolumn{1}{l|}{\priority{100}}    &    -            & Joint  \\ \hline
            2020 & \cite{TOWE-dataset} & Target Opinion Word Extraction (TOWE) & \multicolumn{1}{|p{2cm}|}{\texttt{s}} & \multicolumn{1}{p{3cm}|}{(\textbf{\textit{\color{blue}{pasta}}}, \textbf{\textit{\color{red}{very yummy}}}), (\textbf{\textit{\color{blue}{place}}}, \textbf{\textit{\color{red}{weird smell}}})} & \multicolumn{1}{l|}{-}              & \multicolumn{1}{l|}{-}                 & \priority{-50} & Joint  \\ \hline
            % -    & - & Target Aspect Sentiment Opinion Detection (TASOD) & \multicolumn{1}{l|}{\priority{100}} & \multicolumn{1}{l|}{-}                 & \priority{100} & Joint  \\ \hline
            \end{tabular}%
 }
            \caption{Common sub-tasks of ABSA and their relation with the identified elements (Aspect Categories, Aspect Terms, and Targets). 
            \protect\priority{0}: requires only element detection,
            \protect\priority{50}: requires element detection and sentiment polarity assessment, 
            \protect\priority{-50}: requires element and opinion phrase detection, 
            \protect\priority{100}: requires element, sentiment polarity \& opinion phrase detection,
            \protect\semipriority{50}: requires only sentiment polarity detection for the given element, 
            \textit{single}: task is independent, \textit{Joint}: Task is a multi-task setting or a joint identification task
            }
            \label{tab: Tasks}
            \end{table*}
            
            
            

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


        \begin{table*}[!ht]
        \centering
        \resizebox{0.75\textwidth}{0.55\height}{%
            \begin{tabular}{|p{3cm}|
            % r|
            p{2cm}|lllllllll|lll|p{2.5cm}|}
            \hline
            \multicolumn{1}{|c|}{\multirow{3}{*}{\textbf{\textbf{Dataset Paper}}}} &
            %   \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\textbf{Year}}}} &
              \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Domain}}} &
              \multicolumn{9}{c|}{\textbf{Stats}} &
              \multicolumn{3}{c|}{\textbf{Aspect}} &
              \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Sub-Tasks}}} \\ \cline{3-14}
            \multicolumn{1}{|c|}{} &
              \multicolumn{1}{c|}{} &
             \multicolumn{1}{c|}{\multirow{2}{*}{\#Revs}} &
              \multicolumn{1}{c|}{\multirow{2}{*}{\#Sent}} &
              \multicolumn{1}{c|}{\multirow{2}{*}{IAA}} &
             \multicolumn{3}{c|}{Targ./Term} &
              \multicolumn{3}{c|}{Cat.} &
              \multicolumn{1}{l|}{\textbf{Terms}} &
              \multicolumn{1}{l|}{\textbf{Cat.}} &
              \textbf{Targ.} &
              \multicolumn{1}{c|}{} \\ \cline{6-11}
             
             \multicolumn{1}{|c|}{} &
              \multicolumn{1}{c|}{} &
             \multicolumn{1}{c|}{} &
              \multicolumn{1}{c|}{} &
              \multicolumn{1}{c|}{} &
             \multicolumn{1}{c|}{\#pos} &
              \multicolumn{1}{c|}{\#neg} &
             \multicolumn{1}{c|}{\#neu} &
              \multicolumn{1}{c|}{\#pos} &
              \multicolumn{1}{c|}{\#neg} &
             \multicolumn{1}{c|}{\#neu} &
             \multicolumn{1}{c|}{} &
              \multicolumn{1}{c|}{} &
             \multicolumn{1}{c|}{} &
              \multicolumn{1}{c|}{} \\ \hline
             
            \multicolumn{1}{|c|}{\multirow{5}{*}{\cite{Bing-Liu-Products1}}} &
              %2004 &
              \href{http://www.cs.uic.edu/~liub/FBS/CustomerReviewData.zip}{Cameras} &
            %   34 rev: 346 sents - 203 asp (172 pos, 31 neg) 
\multicolumn{1}{|l|}{34} &
\multicolumn{1}{l|}{346} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{172} &
\multicolumn{1}{l|}{31} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \multicolumn{1}{l|}{-} &
              - &
              ATE, ATSA \\ \cline{2-15}

              \multicolumn{1}{|l|}{} &
            % \cite{Bing-Liu-Products1} &
              %2004 &
              \href{http://www.cs.uic.edu/~liub/FBS/CustomerReviewData.zip}{Phones} &
            %   41 rev: 546 sents - 338 asp (252 pos, 86 neg) 
\multicolumn{1}{|l|}{41} &
\multicolumn{1}{|l|}{546} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{252} &
\multicolumn{1}{l|}{86} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \multicolumn{1}{l|}{-} &
              - &
              ATE, ATSA \\ \cline{2-15}
              
              \multicolumn{1}{|l|}{} &
            % \cite{Bing-Liu-Products1} &
              %2004 &
              \href{http://www.cs.uic.edu/~liub/FBS/CustomerReviewData.zip}{electronics} &
            %   95 rev: 1716 sents - 845 asp (514 pos, 331 neg)
\multicolumn{1}{|l|}{95} &
\multicolumn{1}{|l|}{1716} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{514} &
\multicolumn{1}{l|}{331} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \multicolumn{1}{l|}{-} &
              - &
              ATE, ATSA \\ \cline{2-15}
              
              \multicolumn{1}{|l|}{} &
            % \cite{Bing-Liu-Products1} &
              %2004 &
              \href{http://www.cs.uic.edu/~liub/FBS/CustomerReviewData.zip}{DVD-player} &
            %   99 rev: 739 sents - 430 asp (195 pos, 235 neg) 
\multicolumn{1}{|l|}{99} &
\multicolumn{1}{|l|}{739} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{195} &
\multicolumn{1}{l|}{235} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \multicolumn{1}{l|}{-} &
              - &
              ATE, ATSA \\ \cline{2-15}
              
              \multicolumn{1}{|l|}{} &
            % \cite{Bing-Liu-Products1} &
              %2004 &
              \href{http://www.cs.uic.edu/~liub/FBS/CustomerReviewData.zip}{Cameras} &
            %   45 rev: 597 sents - 285 asp (224 pos, 61 neg) 
\multicolumn{1}{|l|}{45} &
\multicolumn{1}{|l|}{597} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{224} &
\multicolumn{1}{l|}{61} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \multicolumn{1}{l|}{-} &
              - &
              ATE, ATSA \\ \hline
            \multicolumn{1}{|c|}{\multirow{9}{*}{\cite{Bing-Liu-Products2}}} &
              %2008 &
              \href{http://www.cs.uic.edu/~liub/FBS/Reviews-9-products.rar}{Cameras} &
            %   51 rev: 300 sents - 222 asp (164 pos, 58 neg) 
\multicolumn{1}{|l|}{51} &
\multicolumn{1}{|l|}{300} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{164} &
\multicolumn{1}{l|}{58} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \multicolumn{1}{l|}{-} &
              - &
              ATE, ATSA \\ \cline{2-15}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products2} &
              %2008 &
              \href{http://www.cs.uic.edu/~liub/FBS/Reviews-9-products.rar}{Cameras} &
            %   1 rev: 229 sents - 148 asp (121 pos, 27 neg) 
\multicolumn{1}{|l|}{1} &
\multicolumn{1}{|l|}{229} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{121} &
\multicolumn{1}{l|}{27} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \multicolumn{1}{l|}{-} &
              - &
              ATE, ATSA \\ \cline{2-15}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products2} &
              %2008 &
              \href{http://www.cs.uic.edu/~liub/FBS/Reviews-9-products.rar}{Routers} &
            %   31 rev: 312 sents - 265 asp (186 pos, 79 neg) 
\multicolumn{1}{|l|}{31} &
\multicolumn{1}{|l|}{312} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{186} &
\multicolumn{1}{l|}{79} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \multicolumn{1}{l|}{-} &
              - &
              ATE, ATSA \\ \cline{2-15}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products2} &
              %2008 &
              \href{http://www.cs.uic.edu/~liub/FBS/Reviews-9-products.rar}{Phones} &
            %   49 rev: 554 sents - 458 asp (310 pos, 148 neg) 
\multicolumn{1}{|l|}{49} &
\multicolumn{1}{|l|}{594} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{310} &
\multicolumn{1}{l|}{148} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \multicolumn{1}{l|}{-} &
              - &
              ATE, ATSA \\ \cline{2-15}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products2} &
              %2008 &
              \href{http://www.cs.uic.edu/~liub/FBS/Reviews-9-products.rar}{Routers} &
            %   48 rev: 577 sents - 218 asp (154 pos, 64 neg) 
\multicolumn{1}{|l|}{48} &
\multicolumn{1}{|l|}{577} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{154} &
\multicolumn{1}{l|}{64} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \multicolumn{1}{l|}{-} &
              - &
              ATE, ATSA \\ \cline{2-15}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products2} &
              %2008 &
              \href{http://www.cs.uic.edu/~liub/FBS/Reviews-9-products.rar}{Ipod} &
            %   531 sents - 191 asp (129 pos, 62 neg) 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{|l|}{531} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{129} &
\multicolumn{1}{l|}{62} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \multicolumn{1}{l|}{-} &
              - &
              ATE, ATSA \\ \cline{2-15}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products2} &
              %2008 &
              \href{http://www.cs.uic.edu/~liub/FBS/Reviews-9-products.rar}{Mp3 player} &
            %   50 rev: 1011 sents - 583 asp (406 pos, 177 neg) 
\multicolumn{1}{|l|}{50} &
\multicolumn{1}{|l|}{1011} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{406} &
\multicolumn{1}{l|}{177} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \multicolumn{1}{l|}{-} &
              - &
              ATE, ATSA \\ \cline{2-15}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products2} &
              %2008 &
              \href{http://www.cs.uic.edu/~liub/FBS/Reviews-9-products.rar}{Diaper Champ} &
            %   48 rev: 375 sents - 239 asp (183 pos, 56 neg) 
\multicolumn{1}{|l|}{48} &
\multicolumn{1}{|l|}{375} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{183} &
\multicolumn{1}{l|}{56} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \multicolumn{1}{l|}{-} &
              - &
              ATE, ATSA \\ \cline{2-15}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products2} &
              %2008 &
              \href{http://www.cs.uic.edu/~liub/FBS/Reviews-9-products.rar}{Antivirus} &
            %   46 rev: 380 sents - 241 asp (72 pos, 169 neg) 
\multicolumn{1}{|l|}{46} &
\multicolumn{1}{|l|}{380} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{72} &
\multicolumn{1}{l|}{169} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \multicolumn{1}{l|}{-} &
              - &
              ATE, ATSA \\ \hline
            \multicolumn{1}{|c|}{\multirow{2}{*}{\cite{JDPA-Sentiment-Corpus}}} &
              %2010 &
              \href{https://verbs.colorado.edu/jdpacorpus/JDPASentimentCorpus.tar.gz}{Cameras} &
            %   {512 - 19322} 
\multicolumn{1}{|l|}{96} &
\multicolumn{1}{|l|}{3527} &
\multicolumn{1}{l|}{0.85} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \priority{50} &
              TD, TSD \\ \cline{2-15}
            \multicolumn{1}{|c|}{} & % \cite{JDPA-Sentiment-Corpus} &
              %2010 &
              \href{https://verbs.colorado.edu/jdpacorpus/JDPASentimentCorpus.tar.gz}{Cars} &
            %   {512 - 19322} 
\multicolumn{1}{|l|}{111} &
\multicolumn{1}{l|}{4493} &
\multicolumn{1}{l|}{0.85} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \priority{50} &
              TD, TSD \\ \hline
            \multicolumn{1}{|c|}{\multirow{2}{*}{\cite{Darmstadt-Service-Review-Corpus}}} &
              %2010 &
              \href{https://tudatalib.ulb.tu-darmstadt.de/handle/tudatalib/2448}{University reviews} &
            %   {118 - 1151} 
\multicolumn{1}{|l|}{240} &
\multicolumn{1}{l|}{2786} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \priority{50} &
              TD, TSD \\ \cline{2-15}
            \multicolumn{1}{|c|}{} & %\cite{Darmstadt-Service-Review-Corpus} &
              %2010 &
              \href{https://tudatalib.ulb.tu-darmstadt.de/handle/tudatalib/2448}{Service Reviews} &
            %   {118 - 1151} 
\multicolumn{1}{|l|}{234} &
\multicolumn{1}{l|}{6091} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \priority{100} &
              TD, TSD \\ \hline
%             \cite{TripAvisor-AmazonMp3-dataset2} &
%               %2010 &
%               \href{https://www.cs.virginia.edu/~hw5x/dataset.html}{Amazon Mp3} &
               
% &
% \multicolumn{1}{|l|}{-} &
% \multicolumn{1}{l|}{-} &
% \multicolumn{1}{l|}{-} &
% \multicolumn{1}{l|}{-} &
% \multicolumn{1}{l|}{-} &
% \multicolumn{1}{l|}{-} &
% \multicolumn{1}{l|}{-} &
%               \multicolumn{1}{l|}{-} &
%               \multicolumn{1}{l|}{\priority{50}} &
%               - &
%               ACD, ASD, ACSA \\ \hline
            \cite{TripAvisor-AmazonMp3-dataset1} &
              %2011 &
              \href{https://www.cs.virginia.edu/~hw5x/dataset.html}{Trip Advisor**} &
            %   {108891 - 1M} 
            % positive: 1,639,110
            % negative: 153896
            % neutral: 178186
\multicolumn{1}{|l|}{108891} &
\multicolumn{1}{l|}{1M} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{1.63M} &
\multicolumn{1}{l|}{153K} &
\multicolumn{1}{l|}{178K} &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              - &
              ACD, ASD, ACSA \\ \hline
            \multicolumn{1}{|c|}{\multirow{2}{*}{\cite{14-dataset}}} &
              %2014 &
              \href{https://alt.qcri.org/semeval2014/task4/}{Restaurants} &
            %   N - 3841 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{|l|}{3841} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{2892} &
\multicolumn{1}{l|}{1001} &
\multicolumn{1}{l|}{829} &
\multicolumn{1}{l|}{2836} &
\multicolumn{1}{l|}{998} &
\multicolumn{1}{l|}{594} &
              \multicolumn{1}{l|}{\priority{50}} &
              \multicolumn{1}{l|}{\priority{50}} &
              - &
              ATE, ATSA, ACD, ACSA \\ \cline{2-15}
            \multicolumn{1}{|c|}{} & % {\cite{14-dataset}} &
              %2014 &
              \href{https://alt.qcri.org/semeval2014/task4/}{Laptops} &
            %   N - 3845 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{|l|}{3845} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{1331} &
\multicolumn{1}{l|}{994} &
\multicolumn{1}{l|}{629} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \multicolumn{1}{l|}{-} &
              - &
              ATE, ATSA \\ \hline
            \cite{Target-Dependent-Twitter-Sentiment} &
              %2014 &
              \href{http://goo.gl/5Enpu7}{Twitter comments} &
            %   6940 tweets 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{|l|}{6940} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{1734} &
\multicolumn{1}{l|}{1733} &
\multicolumn{1}{l|}{3371} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \priority{50} &
              TD, TSD \\ \hline
            \multicolumn{1}{|c|}{\multirow{3}{*}{\cite{Bing-Liu-Products3}}} &
              %2015 &
              \href{http://www.cs.uic.edu/~liub/FBS/CustomerReviews-3-domains.rar}{Router} &
            %   879 sents - 307 asp (185 pos, 122 neg) 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{879} &
\multicolumn{1}{l|}{0.7} &
\multicolumn{1}{l|}{185} &
\multicolumn{1}{l|}{122} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \multicolumn{1}{l|}{-} &
              - &
              ATE, ATSA \\ \cline{2-15}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products3} &
              %2015 &
              \href{http://www.cs.uic.edu/~liub/FBS/CustomerReviews-3-domains.rar}{Computer} &
            %   581 sents - 354 asp (270 pos, 84 neg) 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{581} &
\multicolumn{1}{l|}{0.7} &
\multicolumn{1}{l|}{270} &
\multicolumn{1}{l|}{84} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \multicolumn{1}{l|}{-} &
              - &
              ATE, ATSA \\ \cline{2-15}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products3} &
              %2015 &
              \href{http://www.cs.uic.edu/~liub/FBS/CustomerReviews-3-domains.rar}{Speaker} &
            %   689 sents - 440 asp (362 pos, 78 neg) 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{689} &
\multicolumn{1}{l|}{0.7} &
\multicolumn{1}{l|}{362} &
\multicolumn{1}{l|}{78} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \multicolumn{1}{l|}{-} &
              - &
              ATE, ATSA \\ \hline
            \multicolumn{1}{|c|}{\multirow{2}{*}{\cite{15-dataset}}} &
              %2015 &
              \href{https://alt.qcri.org/semeval2015/task12/index.php?id=data-and-tools}{Restaurants} &
            %   350 - 2000 
\multicolumn{1}{|l|}{350} &
\multicolumn{1}{l|}{2000} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{1326} &
\multicolumn{1}{l|}{496} &
\multicolumn{1}{l|}{73} &
\multicolumn{1}{l|}{1652} &
\multicolumn{1}{l|}{749} &
\multicolumn{1}{l|}{98} &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \priority{50} &
              TD, TSD, ACD, ASD, TAD, TASD \\ \cline{2-15}
            \multicolumn{1}{|c|}{} & % \cite{15-dataset} &
              %2015 &
              \href{https://alt.qcri.org/semeval2015/task12/index.php?id=data-and-tools}{Laptops} &
            %   450 - 2500 
\multicolumn{1}{|l|}{450} &
\multicolumn{1}{l|}{2500} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{1644} &
\multicolumn{1}{l|}{1094} &
\multicolumn{1}{l|}{185} &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
               &
              ACD, ASD, ACSA \\ \hline
            \multicolumn{1}{|c|}{\multirow{2}{*}{\cite{16-dataset}}} &
              %2016 &
              \href{https://alt.qcri.org/semeval2016/task5/index.php?id=data-and-tools}{Restaurants} &
            %   400 - 2286 
\multicolumn{1}{|l|}{400} &
\multicolumn{1}{l|}{2286} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{1817} &
\multicolumn{1}{l|}{634} &
\multicolumn{1}{l|}{106} &
\multicolumn{1}{l|}{2268} &
\multicolumn{1}{l|}{953} &
\multicolumn{1}{l|}{145} &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \priority{50} &
              TD, TSD, ACD, ASD, TAD, TASD \\ \cline{2-15}
            \multicolumn{1}{|l|}{} & % \multicolumn{1}{|l|}{} & % \cite{16-dataset} &
              %2016 &
              \href{https://alt.qcri.org/semeval2016/task5/index.php?id=data-and-tools}{Laptops} &
            %   530 - 3308 
\multicolumn{1}{|l|}{530} &
\multicolumn{1}{l|}{3308} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{2118} &
\multicolumn{1}{l|}{1358} &
\multicolumn{1}{l|}{236} &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              - &
              ACD, ASD, ACSA \\ \hline
            \cite{sentihood-dataset} &
              %2016 &
              \href{https://github.com/uclnlp/jack/tree/master/data/sentihood}{Urban Neighborhoods} &
            %   N - 5215 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{5215} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{4305} &
\multicolumn{1}{l|}{1606} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \priority{50} &
              TD, TSD, ACD, ASD, TAD, TASD \\ \hline
            \multicolumn{1}{|c|}{\multirow{2}{*}{\cite{BeerAdvocate-TripAdvisor-dataset}}} &
              %2017 &
              \href{https://github.com/HKUST-KnowComp/DMSC}{Beer Advocate**} &
            %   {51020} 
\multicolumn{1}{|l|}{51020} &
\multicolumn{1}{l|}{552K} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{176K} &
\multicolumn{1}{l|}{8902} &
\multicolumn{1}{l|}{64K} &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              - &
              ACD, ASD, ACSA \\ \cline{2-15}
            \multicolumn{1}{|c|}{} & % \cite{BeerAdvocate-TripAdvisor-dataset} &
              %2017 &
              \href{https://github.com/HKUST-KnowComp/DMSC}{Trip Advisor**} &
            %   {29391} 
\multicolumn{1}{|l|}{29391} &
\multicolumn{1}{l|}{375K} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{120K} &
\multicolumn{1}{l|}{66K} &
\multicolumn{1}{l|}{49K} &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              - &
              ACD, ASD, ACSA \\ \hline
            \cite{FiQA-dataset} &
              %2018 &
              \href{https://sites.google.com/view/fiqa/home}{Financial**} &
            %   \begin{tabular}[c]{@{}c@{}}529 headlines \\ 774 microblogs\end{tabular} 
\multicolumn{1}{|l|}{1303} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{774} &
\multicolumn{1}{l|}{399} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{774} &
\multicolumn{1}{l|}{399} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \priority{50} &
              TD, ACD, ASD, TSD, TAD, TASD \\ \hline
            \multicolumn{1}{|c|}{\multirow{2}{*}{\cite{MAMS-dataset}}} &
              %2019 &
              \multicolumn{1}{|c|}{\multirow{2}{*}{\href{https://github.com/siat-nlp/MAMS-for-ABSA/tree/master/data}{Restaurants}}} &
            %   N - 3849 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{3849} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{2415} &
\multicolumn{1}{l|}{2606} &
\multicolumn{1}{l|}{3858} &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              - &
              ACD, ASD, ACSA \\ \cline{3-15}
            \multicolumn{1}{|c|}{} & % \cite{MAMS-dataset} &
              %2019 &
              \multicolumn{1}{|c|}{} &
            %   N - 5297 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{5297} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{4183} &
\multicolumn{1}{l|}{3418} &
\multicolumn{1}{l|}{6253} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              - &
              ATE, ATSA \\ \hline
            \multicolumn{1}{|c|}{\multirow{4}{*}{\cite{TOWE-dataset}}} &
              %2019 &
              Restaurants -14 &
            %   N - 3841 

\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{2127} &
\multicolumn{1}{l|}{-} &
\multicolumn{3}{l|}{3508 targ.- op. pairs} &
% \multicolumn{1}{l|}{-} &
% \multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \priority{-50} &
              TD, TOWE \\ \cline{2-15}
            \multicolumn{1}{|c|}{} & % \cite{TOWE-dataset} &
              %2019 &
              \href{https://github.com/NJUNLP/TOWE/blob/master/data/15res/test.tsv}{Restaurants -15} &
            %   350 - 2000 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{1079} &
\multicolumn{1}{l|}{-} &
\multicolumn{3}{l|}{1512 targ.- op. pairs} &
% \multicolumn{1}{l|}{-} &
% \multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \priority{-50} &
              TD, TOWE \\ \cline{2-15}
            \multicolumn{1}{|c|}{} & % \cite{TOWE-dataset} &
              %2019 &
              \href{https://github.com/NJUNLP/TOWE/blob/master/data/15res/test.tsv}{Restaurants - 16} &
            %   400 - 2286 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{1408} &
\multicolumn{1}{l|}{-} &
\multicolumn{3}{l|}{1969 targ.- op. pairs} &
% \multicolumn{1}{l|}{-} &
% \multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \priority{-50} &
              TD, TOWE \\ \cline{2-15}
            \multicolumn{1}{|c|}{} & % \cite{TOWE-dataset} &
              %2019 &
              \href{https://github.com/NJUNLP/TOWE/blob/master/data/15res/test.tsv}{Laptops - 14} &
            %   N - 3845 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{1501} &
\multicolumn{1}{l|}{-} &
\multicolumn{3}{l|}{2116 targ.- op. pairs} &
% \multicolumn{1}{l|}{-} &
% \multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \priority{-50} &
              TD, TOWE \\ \hline
            \multicolumn{1}{|c|}{\multirow{4}{*}{\cite{ASTE-dataset}}} &
              %2020 &
              \href{https://github.com/xuuuluuu/SemEval-Triplet-data/tree/master/ASTE-Data-V1-AAAI2020}{Restaurants -14} &
            %   N - 3841 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{2119} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{2769} &
\multicolumn{1}{l|}{756} &
\multicolumn{1}{l|}{286} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \priority{100} &
              TD, TOWE, ASTE, TSD \\ \cline{2-15}
            \multicolumn{1}{|c|}{} & % \cite{ASTE-dataset} &
              %2020 &
              \href{https://github.com/xuuuluuu/SemEval-Triplet-data/tree/master/ASTE-Data-V1-AAAI2020}{Restaurants -15} &
            %   350 - 2000 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{1057} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{1285} &
\multicolumn{1}{l|}{401} &
\multicolumn{1}{l|}{61} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \priority{100} &
              TD, TOWE, ASTE, TSD \\ \cline{2-15}
            \multicolumn{1}{|c|}{} & % \cite{ASTE-dataset} &
              %2020 &
              \href{https://github.com/xuuuluuu/SemEval-Triplet-data/tree/master/ASTE-Data-V1-AAAI2020}{Restaurants - 16} &
            %   400 - 2286 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{1372} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{1674} &
\multicolumn{1}{l|}{483} &
\multicolumn{1}{l|}{90} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \priority{100} &
              TD, TOWE, ASTE, TSD \\ \cline{2-15}
            \multicolumn{1}{|c|}{} & % \cite{ASTE-dataset} &
              %2020 &
              \href{https://github.com/xuuuluuu/SemEval-Triplet-data/tree/master/ASTE-Data-V1-AAAI2020}{Laptops - 14} &
            %   N - 3845 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{1487} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{1350} &
\multicolumn{1}{l|}{774} &
\multicolumn{1}{l|}{225} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{-} &
              \priority{100} &
              TD, TOWE, ASTE, TSD \\ \hline
            \end{tabular}%
        }
        \caption{Publicly available English datasets for ABSA and its subtasks. \#R: Number of Reviews, \#S: Number of Sentences. 
        \protect\priority{50}: annotations for the elements and its sentiment polarity are available, 
        \protect\priority{-50}: annotations for the element and its opinion phrase are available, 
        \protect\priority{100}: annotations for the element, its sentiment polarity \& opinion phrase are available. **: indicates that the dataset has ratings converted to categorical sentiment polarities. Note: The domain column has a downloadable link to each dataset.  
        }
        \label{tab: Eng-Datasets}
        \end{table*}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


        \begin{table*}[!ht]
        \centering
        \resizebox{0.85\textwidth}{!}{%
            \begin{tabular}{|p{3cm}|
            % r|
            p{2cm}|lllllllll|p{2.5cm}|}
            \hline
            \multicolumn{1}{|c|}{\multirow{3}{*}{\textbf{\textbf{Dataset Paper}}}} &
            %   \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\textbf{Year}}}} &
              \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Domain}}} &
              \multicolumn{9}{c|}{\textbf{Stats}} &
              \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Sub-Tasks}}} \\ \cline{3-11}
            \multicolumn{1}{|c|}{} &
              \multicolumn{1}{c|}{} &
             \multicolumn{1}{c|}{\multirow{2}{*}{\#Revs}} &
              \multicolumn{1}{c|}{\multirow{2}{*}{\#Sent}} &
              \multicolumn{1}{c|}{\multirow{2}{*}{IAA}} &
             \multicolumn{3}{c|}{Targ./Term} &
              \multicolumn{3}{c|}{Cat.} &
              \multicolumn{1}{c|}{} \\ \cline{6-11}
             
             \multicolumn{1}{|c|}{} &
              \multicolumn{1}{c|}{} &
             \multicolumn{1}{c|}{} &
              \multicolumn{1}{c|}{} &
              \multicolumn{1}{c|}{} &
             \multicolumn{1}{c|}{\#pos} &
              \multicolumn{1}{c|}{\#neg} &
             \multicolumn{1}{c|}{\#neu} &
              \multicolumn{1}{c|}{\#pos} &
              \multicolumn{1}{c|}{\#neg} &
             \multicolumn{1}{c|}{\#neu} &
             \multicolumn{1}{c|}{} \\ \hline
             
            \multicolumn{1}{|c|}{\multirow{5}{*}{\cite{Bing-Liu-Products1}}} &
              %2004 &
              \href{http://www.cs.uic.edu/~liub/FBS/CustomerReviewData.zip}{Cameras} &
            %   34 rev: 346 sents - 203 asp (172 pos, 31 neg) 
\multicolumn{1}{|l|}{34} &
\multicolumn{1}{l|}{346} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{172} &
\multicolumn{1}{l|}{31} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              ATE, ATSA \\ \cline{2-12}

              \multicolumn{1}{|l|}{} &
            % \cite{Bing-Liu-Products1} &
              %2004 &
              \href{http://www.cs.uic.edu/~liub/FBS/CustomerReviewData.zip}{Phones} &
            %   41 rev: 546 sents - 338 asp (252 pos, 86 neg) 
\multicolumn{1}{|l|}{41} &
\multicolumn{1}{|l|}{546} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{252} &
\multicolumn{1}{l|}{86} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              ATE, ATSA \\ \cline{2-12}
              
              \multicolumn{1}{|l|}{} &
            % \cite{Bing-Liu-Products1} &
              %2004 &
              \href{http://www.cs.uic.edu/~liub/FBS/CustomerReviewData.zip}{electronics} &
            %   95 rev: 1716 sents - 845 asp (514 pos, 331 neg)
\multicolumn{1}{|l|}{95} &
\multicolumn{1}{|l|}{1716} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{514} &
\multicolumn{1}{l|}{331} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              ATE, ATSA \\ \cline{2-12}
              
              \multicolumn{1}{|l|}{} &
            % \cite{Bing-Liu-Products1} &
              %2004 &
              \href{http://www.cs.uic.edu/~liub/FBS/CustomerReviewData.zip}{DVD-player} &
            %   99 rev: 739 sents - 430 asp (195 pos, 235 neg) 
\multicolumn{1}{|l|}{99} &
\multicolumn{1}{|l|}{739} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{195} &
\multicolumn{1}{l|}{235} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              ATE, ATSA \\ \cline{2-12}
              
              \multicolumn{1}{|l|}{} &
            % \cite{Bing-Liu-Products1} &
              %2004 &
              \href{http://www.cs.uic.edu/~liub/FBS/CustomerReviewData.zip}{Cameras} &
            %   45 rev: 597 sents - 285 asp (224 pos, 61 neg) 
\multicolumn{1}{|l|}{45} &
\multicolumn{1}{|l|}{597} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{224} &
\multicolumn{1}{l|}{61} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              ATE, ATSA \\ \hline
            \multicolumn{1}{|c|}{\multirow{9}{*}{\cite{Bing-Liu-Products2}}} &
              %2008 &
              \href{http://www.cs.uic.edu/~liub/FBS/Reviews-9-products.rar}{Cameras} &
            %   51 rev: 300 sents - 222 asp (164 pos, 58 neg) 
\multicolumn{1}{|l|}{51} &
\multicolumn{1}{|l|}{300} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{164} &
\multicolumn{1}{l|}{58} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              ATE, ATSA \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products2} &
              %2008 &
              \href{http://www.cs.uic.edu/~liub/FBS/Reviews-9-products.rar}{Cameras} &
            %   1 rev: 229 sents - 148 asp (121 pos, 27 neg) 
\multicolumn{1}{|l|}{1} &
\multicolumn{1}{|l|}{229} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{121} &
\multicolumn{1}{l|}{27} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              ATE, ATSA \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products2} &
              %2008 &
              \href{http://www.cs.uic.edu/~liub/FBS/Reviews-9-products.rar}{Routers} &
            %   31 rev: 312 sents - 265 asp (186 pos, 79 neg) 
\multicolumn{1}{|l|}{31} &
\multicolumn{1}{|l|}{312} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{186} &
\multicolumn{1}{l|}{79} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              ATE, ATSA \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products2} &
              %2008 &
              \href{http://www.cs.uic.edu/~liub/FBS/Reviews-9-products.rar}{Phones} &
            %   49 rev: 554 sents - 458 asp (310 pos, 148 neg) 
\multicolumn{1}{|l|}{49} &
\multicolumn{1}{|l|}{594} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{310} &
\multicolumn{1}{l|}{148} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              ATE, ATSA \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products2} &
              %2008 &
              \href{http://www.cs.uic.edu/~liub/FBS/Reviews-9-products.rar}{Routers} &
            %   48 rev: 577 sents - 218 asp (154 pos, 64 neg) 
\multicolumn{1}{|l|}{48} &
\multicolumn{1}{|l|}{577} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{154} &
\multicolumn{1}{l|}{64} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              ATE, ATSA \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products2} &
              %2008 &
              \href{http://www.cs.uic.edu/~liub/FBS/Reviews-9-products.rar}{Ipod} &
            %   531 sents - 191 asp (129 pos, 62 neg) 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{|l|}{531} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{129} &
\multicolumn{1}{l|}{62} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              ATE, ATSA \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products2} &
              %2008 &
              \href{http://www.cs.uic.edu/~liub/FBS/Reviews-9-products.rar}{Mp3 player} &
            %   50 rev: 1011 sents - 583 asp (406 pos, 177 neg) 
\multicolumn{1}{|l|}{50} &
\multicolumn{1}{|l|}{1011} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{406} &
\multicolumn{1}{l|}{177} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              ATE, ATSA \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products2} &
              %2008 &
              \href{http://www.cs.uic.edu/~liub/FBS/Reviews-9-products.rar}{Diaper Champ} &
            %   48 rev: 375 sents - 239 asp (183 pos, 56 neg) 
\multicolumn{1}{|l|}{48} &
\multicolumn{1}{|l|}{375} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{183} &
\multicolumn{1}{l|}{56} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              ATE, ATSA \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products2} &
              %2008 &
              \href{http://www.cs.uic.edu/~liub/FBS/Reviews-9-products.rar}{Antivirus} &
            %   46 rev: 380 sents - 241 asp (72 pos, 169 neg) 
\multicolumn{1}{|l|}{46} &
\multicolumn{1}{|l|}{380} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{72} &
\multicolumn{1}{l|}{169} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              ATE, ATSA \\ \hline
            \multicolumn{1}{|c|}{\multirow{2}{*}{\cite{JDPA-Sentiment-Corpus}}} &
              %2010 &
              \href{https://verbs.colorado.edu/jdpacorpus/JDPASentimentCorpus.tar.gz}{Cameras} &
            %   {512 - 19322} 
\multicolumn{1}{|l|}{96} &
\multicolumn{1}{|l|}{3527} &
\multicolumn{1}{l|}{0.85} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              TD, TSD \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % \cite{JDPA-Sentiment-Corpus} &
              %2010 &
              \href{https://verbs.colorado.edu/jdpacorpus/JDPASentimentCorpus.tar.gz}{Cars} &
            %   {512 - 19322} 
\multicolumn{1}{|l|}{111} &
\multicolumn{1}{l|}{4493} &
\multicolumn{1}{l|}{0.85} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              TD, TSD \\ \hline
            \multicolumn{1}{|c|}{\multirow{2}{*}{\cite{Darmstadt-Service-Review-Corpus}}} &
              %2010 &
              \href{https://tudatalib.ulb.tu-darmstadt.de/handle/tudatalib/2448}{University reviews} &
            %   {118 - 1151} 
\multicolumn{1}{|l|}{240} &
\multicolumn{1}{l|}{2786} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              TD, TSD \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & %\cite{Darmstadt-Service-Review-Corpus} &
              %2010 &
              \href{https://tudatalib.ulb.tu-darmstadt.de/handle/tudatalib/2448}{Service Reviews} &
            %   {118 - 1151} 
\multicolumn{1}{|l|}{234} &
\multicolumn{1}{l|}{6091} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              TD, TSD \\ \hline
%             \cite{TripAvisor-AmazonMp3-dataset2} &
%               %2010 &
%               \href{https://www.cs.virginia.edu/~hw5x/dataset.html}{Amazon Mp3} &
               
% &
% \multicolumn{1}{|l|}{-} &
% \multicolumn{1}{l|}{-} &
% \multicolumn{1}{l|}{-} &
% \multicolumn{1}{l|}{-} &
% \multicolumn{1}{l|}{-} &
% \multicolumn{1}{l|}{-} &
% \multicolumn{1}{l|}{-} &
%               \multicolumn{1}{l|}{-} &
%               \multicolumn{1}{l|}{\priority{50}} &
%               - &
%               ACD, ASD, ACSA \\ \hline
            \cite{TripAvisor-AmazonMp3-dataset1} &
              %2011 &
              \href{https://www.cs.virginia.edu/~hw5x/dataset.html}{Trip Advisor**} &
            %   {108891 - 1M} 
            % positive: 1,639,110
            % negative: 153896
            % neutral: 178186
\multicolumn{1}{|l|}{108891} &
\multicolumn{1}{l|}{1M} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{1.63M} &
\multicolumn{1}{l|}{153K} &
\multicolumn{1}{l|}{178K} &
              ACD, ASD, ACSA \\ \hline
            \multicolumn{1}{|c|}{\multirow{2}{*}{\cite{14-dataset}}} &
              %2014 &
              \href{https://alt.qcri.org/semeval2014/task4/}{Restaurants} &
            %   N - 3841 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{|l|}{3841} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{2892} &
\multicolumn{1}{l|}{1001} &
\multicolumn{1}{l|}{829} &
\multicolumn{1}{l|}{2836} &
\multicolumn{1}{l|}{998} &
\multicolumn{1}{l|}{594} &
              ATE, ATSA, ACD, ACSA \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % {\cite{14-dataset}} &
              %2014 &
              \href{https://alt.qcri.org/semeval2014/task4/}{Laptops} &
            %   N - 3845 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{|l|}{3845} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{1331} &
\multicolumn{1}{l|}{994} &
\multicolumn{1}{l|}{629} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              ATE, ATSA \\ \hline
            \cite{Target-Dependent-Twitter-Sentiment} &
              %2014 &
              \href{http://goo.gl/5Enpu7}{Twitter comments} &
            %   6940 tweets 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{|l|}{6940} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{1734} &
\multicolumn{1}{l|}{1733} &
\multicolumn{1}{l|}{3371} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              TD, TSD \\ \hline
            \multicolumn{1}{|c|}{\multirow{3}{*}{\cite{Bing-Liu-Products3}}} &
              %2015 &
              \href{http://www.cs.uic.edu/~liub/FBS/CustomerReviews-3-domains.rar}{Router} &
            %   879 sents - 307 asp (185 pos, 122 neg) 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{879} &
\multicolumn{1}{l|}{0.7} &
\multicolumn{1}{l|}{185} &
\multicolumn{1}{l|}{122} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              ATE, ATSA \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products3} &
              %2015 &
              \href{http://www.cs.uic.edu/~liub/FBS/CustomerReviews-3-domains.rar}{Computer} &
            %   581 sents - 354 asp (270 pos, 84 neg) 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{581} &
\multicolumn{1}{l|}{0.7} &
\multicolumn{1}{l|}{270} &
\multicolumn{1}{l|}{84} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              ATE, ATSA \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products3} &
              %2015 &
              \href{http://www.cs.uic.edu/~liub/FBS/CustomerReviews-3-domains.rar}{Speaker} &
            %   689 sents - 440 asp (362 pos, 78 neg) 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{689} &
\multicolumn{1}{l|}{0.7} &
\multicolumn{1}{l|}{362} &
\multicolumn{1}{l|}{78} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              ATE, ATSA \\ \hline
            \multicolumn{1}{|c|}{\multirow{2}{*}{\cite{15-dataset}}} &
              %2015 &
              \href{https://alt.qcri.org/semeval2015/task12/index.php?id=data-and-tools}{Restaurants} &
            %   350 - 2000 
\multicolumn{1}{|l|}{350} &
\multicolumn{1}{l|}{2000} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{1326} &
\multicolumn{1}{l|}{496} &
\multicolumn{1}{l|}{73} &
\multicolumn{1}{l|}{1652} &
\multicolumn{1}{l|}{749} &
\multicolumn{1}{l|}{98} &
              TD, TSD, ACD, ASD, TAD, TASD \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % \cite{15-dataset} &
              %2015 &
              \href{https://alt.qcri.org/semeval2015/task12/index.php?id=data-and-tools}{Laptops} &
            %   450 - 2500 
\multicolumn{1}{|l|}{450} &
\multicolumn{1}{l|}{2500} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{1644} &
\multicolumn{1}{l|}{1094} &
\multicolumn{1}{l|}{185} &
              ACD, ASD, ACSA \\ \hline
            \multicolumn{1}{|c|}{\multirow{2}{*}{\cite{16-dataset}}} &
              %2016 &
              \href{https://alt.qcri.org/semeval2016/task5/index.php?id=data-and-tools}{Restaurants} &
            %   400 - 2286 
\multicolumn{1}{|l|}{400} &
\multicolumn{1}{l|}{2286} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{1817} &
\multicolumn{1}{l|}{634} &
\multicolumn{1}{l|}{106} &
\multicolumn{1}{l|}{2268} &
\multicolumn{1}{l|}{953} &
\multicolumn{1}{l|}{145} &
              TD, TSD, ACD, ASD, TAD, TASD \\ \cline{2-12}
            \multicolumn{1}{|l|}{} & % \multicolumn{1}{|l|}{} & % \cite{16-dataset} &
              %2016 &
              \href{https://alt.qcri.org/semeval2016/task5/index.php?id=data-and-tools}{Laptops} &
            %   530 - 3308 
\multicolumn{1}{|l|}{530} &
\multicolumn{1}{l|}{3308} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{2118} &
\multicolumn{1}{l|}{1358} &
\multicolumn{1}{l|}{236} &
              ACD, ASD, ACSA \\ \hline
            \cite{sentihood-dataset} &
              %2016 &
              \href{https://github.com/uclnlp/jack/tree/master/data/sentihood}{Urban Neighborhoods} &
            %   N - 5215 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{5215} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{4305} &
\multicolumn{1}{l|}{1606} &
\multicolumn{1}{l|}{-} &
              TD, TSD, ACD, ASD, TAD, TASD \\ \hline
            \multicolumn{1}{|c|}{\multirow{2}{*}{\cite{BeerAdvocate-TripAdvisor-dataset}}} &
              %2017 &
              \href{https://github.com/HKUST-KnowComp/DMSC}{Beer Advocate**} &
            %   {51020} 
\multicolumn{1}{|l|}{51020} &
\multicolumn{1}{l|}{552K} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{176K} &
\multicolumn{1}{l|}{8902} &
\multicolumn{1}{l|}{64K} &
              ACD, ASD, ACSA \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % \cite{BeerAdvocate-TripAdvisor-dataset} &
              %2017 &
              \href{https://github.com/HKUST-KnowComp/DMSC}{Trip Advisor**} &
            %   {29391} 
\multicolumn{1}{|l|}{29391} &
\multicolumn{1}{l|}{375K} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{120012} &
\multicolumn{1}{l|}{66017} &
\multicolumn{1}{l|}{49115} &
              ACD, ASD, ACSA \\ \hline
            \cite{FiQA-dataset} &
              %2018 &
              \href{https://sites.google.com/view/fiqa/home}{Financial**} &
            %   \begin{tabular}[c]{@{}c@{}}529 headlines \\ 774 microblogs\end{tabular} 
\multicolumn{1}{|l|}{1303} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{774} &
\multicolumn{1}{l|}{399} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{774} &
\multicolumn{1}{l|}{399} &
\multicolumn{1}{l|}{-} &
              TD, ACD, ASD, TSD, TAD, TASD \\ \hline
            \multicolumn{1}{|c|}{\multirow{2}{*}{\cite{MAMS-dataset}}} &
              %2019 &
              \multicolumn{1}{|c|}{\multirow{2}{*}{\href{https://github.com/siat-nlp/MAMS-for-ABSA/tree/master/data}{Restaurants}}} &
            %   N - 3849 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{3849} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{2415} &
\multicolumn{1}{l|}{2606} &
\multicolumn{1}{l|}{3858} &
              ACD, ASD, ACSA \\ \cline{3-12}
            \multicolumn{1}{|c|}{} & % \cite{MAMS-dataset} &
              %2019 &
              \multicolumn{1}{|c|}{} &
            %   N - 5297 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{5297} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{4183} &
\multicolumn{1}{l|}{3418} &
\multicolumn{1}{l|}{6253} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              ATE, ATSA \\ \hline
            \multicolumn{1}{|c|}{\multirow{4}{*}{\cite{TOWE-dataset}}} &
              %2019 &
              Restaurants -14 &
            %   N - 3841 

\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{2127} &
\multicolumn{1}{l|}{-} &
\multicolumn{3}{l|}{3508 targ.- op. pairs} &
% \multicolumn{1}{l|}{-} &
% \multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              TD, TOWE \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % \cite{TOWE-dataset} &
              %2019 &
              \href{https://github.com/NJUNLP/TOWE/blob/master/data/15res/test.tsv}{Restaurants -15} &
            %   350 - 2000 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{1079} &
\multicolumn{1}{l|}{-} &
\multicolumn{3}{l|}{1512 targ.- op. pairs} &
% \multicolumn{1}{l|}{-} &
% \multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              TD, TOWE \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % \cite{TOWE-dataset} &
              %2019 &
              \href{https://github.com/NJUNLP/TOWE/blob/master/data/15res/test.tsv}{Restaurants - 16} &
            %   400 - 2286 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{1408} &
\multicolumn{1}{l|}{-} &
\multicolumn{3}{l|}{1969 targ.- op. pairs} &
% \multicolumn{1}{l|}{-} &
% \multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              TD, TOWE \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % \cite{TOWE-dataset} &
              %2019 &
              \href{https://github.com/NJUNLP/TOWE/blob/master/data/15res/test.tsv}{Laptops - 14} &
            %   N - 3845 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{1501} &
\multicolumn{1}{l|}{-} &
\multicolumn{3}{l|}{2116 targ.- op. pairs} &
% \multicolumn{1}{l|}{-} &
% \multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              TD, TOWE \\ \hline
            \multicolumn{1}{|c|}{\multirow{4}{*}{\cite{ASTE-dataset}}} &
              %2020 &
              \href{https://github.com/xuuuluuu/SemEval-Triplet-data/tree/master/ASTE-Data-V1-AAAI2020}{Restaurants -14} &
            %   N - 3841 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{2119} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{2769} &
\multicolumn{1}{l|}{756} &
\multicolumn{1}{l|}{286} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              TD, TOWE, ASTE, TSD \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % \cite{ASTE-dataset} &
              %2020 &
              \href{https://github.com/xuuuluuu/SemEval-Triplet-data/tree/master/ASTE-Data-V1-AAAI2020}{Restaurants -15} &
            %   350 - 2000 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{1057} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{1285} &
\multicolumn{1}{l|}{401} &
\multicolumn{1}{l|}{61} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              TD, TOWE, ASTE, TSD \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % \cite{ASTE-dataset} &
              %2020 &
              \href{https://github.com/xuuuluuu/SemEval-Triplet-data/tree/master/ASTE-Data-V1-AAAI2020}{Restaurants - 16} &
            %   400 - 2286 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{1372} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{1674} &
\multicolumn{1}{l|}{483} &
\multicolumn{1}{l|}{90} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              TD, TOWE, ASTE, TSD \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % \cite{ASTE-dataset} &
              %2020 &
              \href{https://github.com/xuuuluuu/SemEval-Triplet-data/tree/master/ASTE-Data-V1-AAAI2020}{Laptops - 14} &
            %   N - 3845 
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{1487} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{1350} &
\multicolumn{1}{l|}{774} &
\multicolumn{1}{l|}{225} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
              TD, TOWE, ASTE, TSD \\ \hline
            \end{tabular}%
        }
        \caption{Publicly available English datasets for ABSA and its subtasks. \#R: Number of Reviews, \#S: Number of Sentences. 
        **: indicates that the dataset has ratings converted to categorical sentiment polarities. Note: The domain column has a downloadable link to each dataset.  
        }
        \label{tab: Eng-Datasets}
        \end{table*}




% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




        \begin{table*}[!ht]
        \centering
        \resizebox{\textwidth}{!}{%
            \begin{tabular}{|p{3cm}|
            % l|
            l|l|p{6cm}|lll|l|}
            \hline
            \multirow{2}{3cm}{\textbf{Dataset Paper}} &
            %   \multirow{2}{*}{\textbf{Year}} &
              \multirow{2}{*}{\textbf{Language}} &
              \multirow{2}{*}{\textbf{Domain}} &
              \multirow{2}{*}{\textbf{\#R - \#S}} &
              \multicolumn{3}{c|}{\textbf{Aspect}} &
              \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Related \\ Sub-Tasks\end{tabular}}} \\ \cline{5-7}
             &
            %   &
               &
               &
               &
              \multicolumn{1}{l|}{\textbf{Terms}} &
              \multicolumn{1}{l|}{\textbf{Cat.}} &
              \textbf{Targ.} &
               \\ \hline
            \cite{Arabic-book} &
              %2015 &
              Arabic &
              \href{https://github.com/msmadi/HAAD}{Books} &
              N - 1513 &
              \multicolumn{1}{l|}{\priority{50}} &
              \multicolumn{1}{l|}{\priority{50}} &
              - &
              ATE, ATSA, ACD, ACSA \\ \hline
            \multicolumn{1}{|l|}{\multirow{9}{3cm}{\cite{16-dataset}}} &
              %2016 &
              Spanish &
              \href{https://alt.qcri.org/semeval2016/task5/index.php?id=data-and-tools}{Restaurants} &
              N - 2691 &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \priority{50} &
              TD, TSD, ACD, ASD, TAD, TASD \\ \cline{2-8}
            \multicolumn{1}{|l|}{} & % \cite{16-dataset} &
              %2016 &
              Turkish &
              \href{https://alt.qcri.org/semeval2016/task5/index.php?id=data-and-tools}{Restaurants} &
              300 - N &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \priority{50} &
              TD, TSD, ACD, ASD, TAD, TASD \\ \cline{2-8}
            \multicolumn{1}{|l|}{} & % \cite{16-dataset} &
              %2016 &
              Turkish &
              \href{https://alt.qcri.org/semeval2016/task5/index.php?id=data-and-tools}{Telecom} &
              3000 - N &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \priority{50} &
              TD, TSD, ACD, ASD, TAD, TASD \\ \cline{2-8}
            \multicolumn{1}{|l|}{} & % \cite{16-dataset} &
              %2016 &
              Arabic &
              \href{https://alt.qcri.org/semeval2016/task5/index.php?id=data-and-tools}{Hotels} &
              3000 - 6000 &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \priority{50} &
              TD, TSD, ACD, ASD, TAD, TASD \\ \cline{2-8}
            \multicolumn{1}{|l|}{} & % \cite{16-dataset} &
              %2016 &
              Dutch &
              \href{https://alt.qcri.org/semeval2016/task5/index.php?id=data-and-tools}{Restaurants} &
              400 - 2297 &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \priority{50} &
              TD, TSD, ACD, ASD, TAD, TASD \\ \cline{2-8}
            \multicolumn{1}{|l|}{} & % \cite{16-dataset} &
              %2016 &
              Dutch &
              \href{https://alt.qcri.org/semeval2016/task5/index.php?id=data-and-tools}{Mobile Phones} &
              270 - 1697 &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              - &
              ACD, ASD, ACSA \\ \cline{2-8}
            \multicolumn{1}{|l|}{} & % \cite{16-dataset} &
              %2016 &
              Russian &
              \href{https://alt.qcri.org/semeval2016/task5/index.php?id=data-and-tools}{Restaurants} &
              300 - 4000 &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \priority{50} &
              TD, TSD, ACD, ASD, TAD, TASD \\ \cline{2-8}
            \multicolumn{1}{|l|}{} & % \cite{16-dataset} &
              %2016 &
              French &
              \href{https://alt.qcri.org/semeval2016/task5/index.php?id=data-and-tools}{Restaurants} &
              470 - 2500 &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              \priority{50} &
              TD, TSD, ACD, ASD, TAD, TASD \\ \cline{2-8}
            \multicolumn{1}{|l|}{} & % \cite{16-dataset} &
              %2016 &
              Chinese &
              \href{https://alt.qcri.org/semeval2016/task5/index.php?id=data-and-tools}{\begin{tabular}[c]{@{}l@{}}Mobile Phones \\ Digital Cameras\end{tabular}} &
              400 - 4100 &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              - &
              ACD, ASD, ACSA \\ \hline
            \multicolumn{1}{|l|}{\multirow{2}{3cm}{\cite{Bangla}}} &
              %2018 &
              Bangla &
              \href{https://github.com/AtikRahman/Bangla_ABSA_Datasets}{Cricket} &
              N - 2691 &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              - &
              ACD, ACSA, ASD \\ \cline{2-8}
            \multicolumn{1}{|c|}{} & % \cite{Bangla} &
              %2018 &
              Bangla &
              \href{https://github.com/AtikRahman/Bangla_ABSA_Datasets}{Restaurants} &
              N - 1712 &
              \multicolumn{1}{l|}{-} &
              \multicolumn{1}{l|}{\priority{50}} &
              - &
              ACD, ACSA, ASD \\ \hline
            \cite{char-CNN-Chin} &
              %2018 &
              Chinese &
              Automobile &
               &
              \multicolumn{1}{l|}{\priority{50}} &
              \multicolumn{1}{l|}{\priority{50}} &
              - &
              ATE, ATSA, ACD, ACSA, ASD \\ \hline
            \cite{telugu-dataset} &
              %2020 &
              Telugu &
              \href{http://tiny.cc/vdxugz}{Movies} &
              N - 5027 &
              \multicolumn{1}{l|}{\priority{50}} &
              \multicolumn{1}{l|}{\priority{50}} &
              - &
              ATE, ATSA, ACD, ACSA \\ \hline
              \cite{chinese-rest-asap-2021} &
              %2018 &
              Chinese &
              \href{https://github.com/Meituan-Dianping/asap/tree/master/data}{Restaurants} &
               &
              - &
              \multicolumn{1}{|l|}{\priority{50}} &
              - &
              ACD, ACSA, ASD \\ \hline
            \end{tabular}%
        }
        \caption{Publicly available Other language datasets for ABSA and its subtasks. \#R: Number of Reviews, \#S: Number of Sentences. 
        \protect\priority{50}: annotations for the element and its sentiment polarity are available.
        }
        \label{tab: Non-Eng-Datasets}
        \end{table*}





% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        \begin{table*}[!ht]
        \centering
        \resizebox{0.9\textwidth}{0.52\height}{%
            \begin{tabular}{|p{2cm}|
            % r|
            p{3cm}|p{2.5cm}|lllllllll|}
            \hline
            \multicolumn{1}{|l|}{\multirow{3}{*}{\textbf{\textbf{Dataset Paper}}}} &
            %   \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\textbf{Year}}}} &
              \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Source}}} &
              \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Domain}}} &
              \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Lang}}} &
              \multicolumn{8}{c|}{\textbf{Stats}} \\ \cline{5-12}
            \multicolumn{1}{|c|}{} &
              \multicolumn{1}{c|}{} &
              \multicolumn{1}{c|}{} &
              \multicolumn{1}{c|}{} &
             \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\#Revs}}} &
              \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\#Sent}}} &
             \multicolumn{3}{c|}{\textbf{Target/Aspect Term}} &
              \multicolumn{3}{c|}{\textbf{Aspect Categor}y} \\ \cline{7-12}
             
             \multicolumn{1}{|c|}{} &
              \multicolumn{1}{c|}{} &
              \multicolumn{1}{c|}{} &
             \multicolumn{1}{c|}{} &
              \multicolumn{1}{c|}{} &
              \multicolumn{1}{c|}{} &
             \multicolumn{1}{c|}{\#pos} &
              \multicolumn{1}{c|}{\#neg} &
             \multicolumn{1}{c|}{\#neu} &
              \multicolumn{1}{c|}{\#pos} &
              \multicolumn{1}{c|}{\#neg} &
             \multicolumn{1}{c|}{\#neu} \\ \hline
             
            \multicolumn{1}{|l|}{\multirow{5}{2.5cm}{Customer Reviews \cite{Bing-Liu-Products1}}} &
              %2004 &
              \multicolumn{1}{|l|}{\multirow{5}{2.5cm}{Amazon.com}}  & 
              \href{http://www.cs.uic.edu/~liub/FBS/CustomerReviewData.zip}{Cameras} &
            %   34 rev: 346 sents - 203 asp (172 pos, 31 neg) 
            English &
\multicolumn{1}{|l|}{34} &
\multicolumn{1}{l|}{346} &
\multicolumn{1}{l|}{172} &
\multicolumn{1}{l|}{31} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \cline{3-12}

              \multicolumn{1}{|l|}{} &
            % \cite{Bing-Liu-Products1} &
              %2004 &
              &
              \href{http://www.cs.uic.edu/~liub/FBS/CustomerReviewData.zip}{Phones} &
            %   41 rev: 546 sents - 338 asp (252 pos, 86 neg) 
            English &
\multicolumn{1}{|l|}{41} &
\multicolumn{1}{|l|}{546} &
\multicolumn{1}{l|}{252} &
\multicolumn{1}{l|}{86} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \cline{3-12}
              
              \multicolumn{1}{|l|}{} &
            % \cite{Bing-Liu-Products1} &
              %2004 &
              &
              \href{http://www.cs.uic.edu/~liub/FBS/CustomerReviewData.zip}{Electronics} &
            %   95 rev: 1716 sents - 845 asp (514 pos, 331 neg)
            English &
\multicolumn{1}{|l|}{95} &
\multicolumn{1}{|l|}{1716} &
\multicolumn{1}{l|}{514} &
\multicolumn{1}{l|}{331} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \cline{3-12}
              
              \multicolumn{1}{|l|}{} &
            % \cite{Bing-Liu-Products1} &
              %2004 &
              &
              \href{http://www.cs.uic.edu/~liub/FBS/CustomerReviewData.zip}{DVD-player} &
            %   99 rev: 739 sents - 430 asp (195 pos, 235 neg) 
            English &
\multicolumn{1}{|l|}{99} &
\multicolumn{1}{|l|}{739} &
\multicolumn{1}{l|}{195} &
\multicolumn{1}{l|}{235} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \cline{3-12}
              
              \multicolumn{1}{|l|}{} &
            % \cite{Bing-Liu-Products1} &
              %2004 &
              &
              \href{http://www.cs.uic.edu/~liub/FBS/CustomerReviewData.zip}{Cameras} &
            %   45 rev: 597 sents - 285 asp (224 pos, 61 neg) 
            English &
\multicolumn{1}{|l|}{45} &
\multicolumn{1}{|l|}{597} &
\multicolumn{1}{l|}{224} &
\multicolumn{1}{l|}{61} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \hline
            \multicolumn{1}{|l|}{\multirow{9}{2.5cm}{Customer Reviews \cite{Bing-Liu-Products2}}} &
              %2008 &
              \multicolumn{1}{|l|}{\multirow{9}{2.5cm}{Amazon.com}} &
              \href{http://www.cs.uic.edu/~liub/FBS/Reviews-9-products.rar}{Cameras} &
            %   51 rev: 300 sents - 222 asp (164 pos, 58 neg) 
            English &
\multicolumn{1}{|l|}{51} &
\multicolumn{1}{|l|}{300} &
\multicolumn{1}{l|}{164} &
\multicolumn{1}{l|}{58} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \cline{3-12}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products2} &
              %2008 &
              &
              \href{http://www.cs.uic.edu/~liub/FBS/Reviews-9-products.rar}{Cameras} &
            %   1 rev: 229 sents - 148 asp (121 pos, 27 neg) 
            English &
\multicolumn{1}{|l|}{1} &
\multicolumn{1}{|l|}{229} &
\multicolumn{1}{l|}{121} &
\multicolumn{1}{l|}{27} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \cline{3-12}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products2} &
              %2008 &
              &
              \href{http://www.cs.uic.edu/~liub/FBS/Reviews-9-products.rar}{Routers} &
            %   31 rev: 312 sents - 265 asp (186 pos, 79 neg) 
            English &
\multicolumn{1}{|l|}{31} &
\multicolumn{1}{|l|}{312} &
\multicolumn{1}{l|}{186} &
\multicolumn{1}{l|}{79} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \cline{3-12}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products2} &
              %2008 &
              &
              \href{http://www.cs.uic.edu/~liub/FBS/Reviews-9-products.rar}{Phones} &
            %   49 rev: 554 sents - 458 asp (310 pos, 148 neg) 
            English &
\multicolumn{1}{|l|}{49} &
\multicolumn{1}{|l|}{594} &
\multicolumn{1}{l|}{310} &
\multicolumn{1}{l|}{148} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \cline{3-12}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products2} &
              %2008 &
              &
              \href{http://www.cs.uic.edu/~liub/FBS/Reviews-9-products.rar}{Routers} &
            %   48 rev: 577 sents - 218 asp (154 pos, 64 neg) 
            English &
\multicolumn{1}{|l|}{48} &
\multicolumn{1}{|l|}{577} &
\multicolumn{1}{l|}{154} &
\multicolumn{1}{l|}{64} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \cline{3-12}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products2} &
              %2008 &
              &
              \href{http://www.cs.uic.edu/~liub/FBS/Reviews-9-products.rar}{Ipod} &
            %   531 sents - 191 asp (129 pos, 62 neg) 
            English &
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{|l|}{531} &
\multicolumn{1}{l|}{129} &
\multicolumn{1}{l|}{62} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \cline{3-12}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products2} &
              %2008 &
              &
              \href{http://www.cs.uic.edu/~liub/FBS/Reviews-9-products.rar}{Mp3 player} &
            %   50 rev: 1011 sents - 583 asp (406 pos, 177 neg) 
            English &
\multicolumn{1}{|l|}{50} &
\multicolumn{1}{|l|}{1011} &
\multicolumn{1}{l|}{406} &
\multicolumn{1}{l|}{177} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \cline{3-12}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products2} &
              %2008 &
              &
              \href{http://www.cs.uic.edu/~liub/FBS/Reviews-9-products.rar}{Diaper Champ} &
            %   48 rev: 375 sents - 239 asp (183 pos, 56 neg) 
            English &
\multicolumn{1}{|l|}{48} &
\multicolumn{1}{|l|}{375} &
\multicolumn{1}{l|}{183} &
\multicolumn{1}{l|}{56} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \cline{3-12}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products2} &
              %2008 &
              &
              \href{http://www.cs.uic.edu/~liub/FBS/Reviews-9-products.rar}{Antivirus} &
            %   46 rev: 380 sents - 241 asp (72 pos, 169 neg) 
            English &
\multicolumn{1}{|l|}{46} &
\multicolumn{1}{|l|}{380} &
\multicolumn{1}{l|}{72} &
\multicolumn{1}{l|}{169} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \hline
            \multicolumn{1}{|l|}{\multirow{2}{2.5cm}{JDPA \cite{JDPA-Sentiment-Corpus}}} &
              %2010 &
              \multicolumn{1}{|l|}{\multirow{2}{2.5cm}{J.D. Power and Associates}} & 
              \href{https://verbs.colorado.edu/jdpacorpus/JDPASentimentCorpus.tar.gz}{Cameras} &
            %   {512 - 19322} 
            English &
\multicolumn{1}{|l|}{96} &
\multicolumn{1}{|l|}{3527} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \cline{3-12}
            \multicolumn{1}{|c|}{} & % \cite{JDPA-Sentiment-Corpus} &
              %2010 &
              & 
              \href{https://verbs.colorado.edu/jdpacorpus/JDPASentimentCorpus.tar.gz}{Cars} &
            %   {512 - 19322} 
            English &
\multicolumn{1}{|l|}{111} &
\multicolumn{1}{l|}{4493} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \hline
            \multicolumn{1}{|l|}{\multirow{2}{2.5cm}{Darmstadt Service \cite{Darmstadt-Service-Review-Corpus}}} &
              %2010 &
              tu-darmstadt.de & 
              \href{https://tudatalib.ulb.tu-darmstadt.de/handle/tudatalib/2448}{University reviews} &
            %   {118 - 1151} 
            English &
\multicolumn{1}{|l|}{240} &
\multicolumn{1}{l|}{2786} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & %\cite{Darmstadt-Service-Review-Corpus} &
              %2010 &
              Darmstadt car service & 
              \href{https://tudatalib.ulb.tu-darmstadt.de/handle/tudatalib/2448}{Service Reviews} &
            %   {118 - 1151} 
            English &
\multicolumn{1}{|l|}{234} &
\multicolumn{1}{l|}{6091} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \hline
%             \cite{TripAvisor-AmazonMp3-dataset2} &
%               %2010 &
%               \href{https://www.cs.virginia.edu/~hw5x/dataset.html}{Amazon Mp3} &
               
% &
% \multicolumn{1}{|l|}{-} &
% \multicolumn{1}{l|}{-} &
% \multicolumn{1}{l|}{-} &
% \multicolumn{1}{l|}{-} &
% \multicolumn{1}{l|}{-} &
% \multicolumn{1}{l|}{-} &
% \multicolumn{1}{l|}{-} &
%               \multicolumn{1}{l|}{-} &
%               \multicolumn{1}{l|}{\priority{50}} &
%               - &
%               ACD, ASD, ACSA \\ \hline
            Twitter Comments \cite{Target-Dependent-Twitter-Sentiment} &
              %2014 &
              www.twitter.com & 
              \href{http://goo.gl/5Enpu7}{Twitter comments} &
            %   6940 tweets 
            English &
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{|l|}{6940} &
\multicolumn{1}{l|}{1734} &
\multicolumn{1}{l|}{1733} &
\multicolumn{1}{l|}{3371} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \hline
            \multicolumn{1}{|l|}{\multirow{1}{2.5cm}{SE-14 \cite{14-dataset}}} &
             %2014 &
              Amazon.com & 
              \href{https://alt.qcri.org/semeval2014/task4/}{Laptops} &
            %   N - 3845 
            English &
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{|l|}{3845} &
\multicolumn{1}{l|}{1331} &
\multicolumn{1}{l|}{994} &
\multicolumn{1}{l|}{629} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \hline
            \multicolumn{1}{|l|}{\multirow{3}{2.5cm}{Customer Reviews \cite{Bing-Liu-Products3}}} &
              %2015 &
              \multicolumn{1}{|l|}{\multirow{3}{2.5cm}{Amazon.com}} & 
              \href{http://www.cs.uic.edu/~liub/FBS/CustomerReviews-3-domains.rar}{Router} &
            %   879 sents - 307 asp (185 pos, 122 neg) 
            English &
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{879} &
\multicolumn{1}{l|}{185} &
\multicolumn{1}{l|}{122} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \cline{3-12}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products3} &
              %2015 &
               & 
              \href{http://www.cs.uic.edu/~liub/FBS/CustomerReviews-3-domains.rar}{Computer} &
            %   581 sents - 354 asp (270 pos, 84 neg) 
            English &
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{581} &
\multicolumn{1}{l|}{270} &
\multicolumn{1}{l|}{84} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \cline{3-12}
            \multicolumn{1}{|c|}{} & % \cite{Bing-Liu-Products3} &
              %2015 &
               & 
              \href{http://www.cs.uic.edu/~liub/FBS/CustomerReviews-3-domains.rar}{Speaker} &
            %   689 sents - 440 asp (362 pos, 78 neg) 
            English &
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{689} &
\multicolumn{1}{l|}{362} &
\multicolumn{1}{l|}{78} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \hline
            \multicolumn{1}{|l|}{\multirow{1}{2.5cm}{MAMS \cite{MAMS-dataset}}} &
              %2019 &
              & 
              \multicolumn{1}{|c|}{} &

            %   N - 5297 
            English &
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{5297} &
\multicolumn{1}{l|}{4183} &
\multicolumn{1}{l|}{3418} &
\multicolumn{1}{l|}{6253} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \hline
            \multicolumn{1}{|l|}{\multirow{4}{2.5cm}{TOWE \cite{TOWE-dataset}}} &
              %2019 &
              SE-14 Restaurants & 
              \href{https://github.com/NJUNLP/TOWE/blob/master/data/14res/test.tsv}{Restaurants\textsuperscript{\pm\pm}} &

            %   N - 3841 

            English &
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{2127} &
\multicolumn{3}{l|}{3508 targ.- op. pairs} &
% \multicolumn{1}{l|}{-} &
% \multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % \cite{TOWE-dataset} &
              %2019 &
              SE-15 Restaurants & 
              \href{https://github.com/NJUNLP/TOWE/blob/master/data/15res/test.tsv}{Restaurants\textsuperscript{\pm\pm}} &
            %   350 - 2000 
            English &
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{1079} &
\multicolumn{3}{l|}{1512 targ.- op. pairs} &
% \multicolumn{1}{l|}{-} &
% \multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % \cite{TOWE-dataset} &
              %2019 &
              SE-16 Restaurants & 
              \href{https://github.com/NJUNLP/TOWE/blob/master/data/15res/test.tsv}{Restaurants\textsuperscript{\pm\pm}} &
            %   400 - 2286 
            English &
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{1408} &
\multicolumn{3}{l|}{1969 targ.- op. pairs} &
% \multicolumn{1}{l|}{-} &
% \multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % \cite{TOWE-dataset} &
              %2019 &
              SE-14 Laptops & 
              \href{https://github.com/NJUNLP/TOWE/blob/master/data/15res/test.tsv}{Laptops\textsuperscript{\pm\pm}} &
            %   N - 3845 
            English &
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{1501} &
\multicolumn{3}{l|}{2116 targ.- op. pairs} &
% \multicolumn{1}{l|}{-} &
% \multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \hline
            \multicolumn{1}{|l|}{\multirow{4}{2.5cm}{\cite{telugu-dataset}}} &
              %2020 &
              \href{123telugu.com}{123telugu}, \href{eenadu.net}{eenadu}, \href{telugu.samayam.com}{samayam} &
              \href{http://tiny.cc/vdxugz}{Movies} &
              Telugu &
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{5027} &
\multicolumn{1}{l|}{2480} &
\multicolumn{1}{l|}{3251} &
\multicolumn{1}{l|}{1129} &
\multicolumn{1}{l|}{2480} &
\multicolumn{1}{l|}{3251} &
\multicolumn{1}{l|}{1129} \\ \hline
            \multicolumn{1}{|l|}{\multirow{4}{2.5cm}{ASTE \cite{ASTE-dataset}}} &
              %2020 &
              SE-14 Restaurants & 
              \href{https://github.com/xuuuluuu/SemEval-Triplet-data/tree/master/ASTE-Data-V1-AAAI2020}{Restaurants\textsuperscript{\pm\pm}} &
            %   N - 3841 
            English &
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{2119} &
\multicolumn{1}{l|}{2769} &
\multicolumn{1}{l|}{756} &
\multicolumn{1}{l|}{286} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % \cite{ASTE-dataset} &
              %2020 &
              SE-15 Restaurants & 
              \href{https://github.com/xuuuluuu/SemEval-Triplet-data/tree/master/ASTE-Data-V1-AAAI2020}{Restaurants\textsuperscript{\pm\pm}} &
            %   350 - 2000 
            English &
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{1057} &
\multicolumn{1}{l|}{1285} &
\multicolumn{1}{l|}{401} &
\multicolumn{1}{l|}{61} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % \cite{ASTE-dataset} &
              %2020 &
              SE-16 Restaurants & 
              \href{https://github.com/xuuuluuu/SemEval-Triplet-data/tree/master/ASTE-Data-V1-AAAI2020}{Restaurants\textsuperscript{\pm\pm}} &
            %   400 - 2286 
            English &
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{1372} &
\multicolumn{1}{l|}{1674} &
\multicolumn{1}{l|}{483} &
\multicolumn{1}{l|}{90} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % \cite{ASTE-dataset} &
              %2020 &
              SE-14 Laptops & 
              \href{https://github.com/xuuuluuu/SemEval-Triplet-data/tree/master/ASTE-Data-V1-AAAI2020}{Laptops\textsuperscript{\pm\pm}} &
            %   N - 3845 
            English &
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{1487} &
\multicolumn{1}{l|}{1350} &
\multicolumn{1}{l|}{774} &
\multicolumn{1}{l|}{225} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \hline
            \end{tabular}%
        }
        \caption{Publicly available English datasets for ABSA and its subtasks. Lang.: Language, \#R: Number of Reviews, \#S: Number of Sentences. 
        **: indicates that the dataset has ratings converted to categorical sentiment polarities. Note: The domain column has a downloadable link to each dataset.  
        $\pm\pm$: indicates that those datasets have the opinion phrase annotation along with other elements.
        }
        \label{tab: Eng-Datasets}
        \end{table*}





% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



        \begin{table*}[!ht]
        \centering
        \resizebox{0.9\textwidth}{0.52\height}{%
            \begin{tabular}{|p{2cm}|
            % r|
            p{3cm}|p{2.5cm}|lllllllll|}
            \hline
            \multicolumn{1}{|l|}{\multirow{3}{*}{\textbf{\textbf{Dataset Paper}}}} &
            %   \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\textbf{Year}}}} &
              \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Source}}} &
              \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Domain}}} &
              \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Lang}}} &
              \multicolumn{8}{c|}{\textbf{Stats}} \\ \cline{5-12}
            \multicolumn{1}{|c|}{} &
              \multicolumn{1}{c|}{} &
              \multicolumn{1}{c|}{} &
              \multicolumn{1}{c|}{} &
             \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\#Revs}}} &
              \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\#Sent}}} &
             \multicolumn{3}{c|}{\textbf{Target/Aspect Term}} &
              \multicolumn{3}{c|}{\textbf{Aspect Categor}y} \\ \cline{7-12}
             
             \multicolumn{1}{|c|}{} &
              \multicolumn{1}{c|}{} &
              \multicolumn{1}{c|}{} &
             \multicolumn{1}{c|}{} &
              \multicolumn{1}{c|}{} &
              \multicolumn{1}{c|}{} &
             \multicolumn{1}{c|}{\#pos} &
              \multicolumn{1}{c|}{\#neg} &
             \multicolumn{1}{c|}{\#neu} &
              \multicolumn{1}{c|}{\#pos} &
              \multicolumn{1}{c|}{\#neg} &
             \multicolumn{1}{c|}{\#neu} \\ \hline
             
            TripAdvisor Hotels \cite{TripAvisor-AmazonMp3-dataset1} &
              %2011 &
              \multicolumn{1}{|l|}{\multirow{2}{2.5cm}{www.tripadvisor.com}} &
              \href{https://www.cs.virginia.edu/~hw5x/dataset.html}{Hotels**} &
            %   {108891 - 1M} 
            % positive: 1,639,110
            % negative: 153896
            % neutral: 178186
            English &
\multicolumn{1}{|l|}{108891} &
\multicolumn{1}{l|}{1M} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{1.63M} &
\multicolumn{1}{l|}{153K} &
\multicolumn{1}{l|}{178K} \\ \hline
            \multicolumn{1}{|l|}{\multirow{1}{2.5cm}{SE-14 \cite{14-dataset}}} &
              %2014 &
              CitySearch New York \cite{Ganu-CitySearch} & 
              \href{https://alt.qcri.org/semeval2014/task4/}{Restaurants} &
            %   N - 3841 
            English &
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{|l|}{3841} &
\multicolumn{1}{l|}{2892} &
\multicolumn{1}{l|}{1001} &
\multicolumn{1}{l|}{829} &
\multicolumn{1}{l|}{2836} &
\multicolumn{1}{l|}{998} &
\multicolumn{1}{l|}{594} \\ \hline
            \multicolumn{1}{|l|}{\multirow{2}{3cm}{HAAD \cite{Arabic-book}}} &
              %2015 &
              LABR book reviews & 
              \href{https://alt.qcri.org/semeval2015/task12/index.php?id=data-and-tools}{Restaurants} &
            %   350 - 2000 
            English &
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{2389} &
\multicolumn{1}{l|}{1376} &
\multicolumn{1}{l|}{1287} &
\multicolumn{1}{l|}{148} &
\multicolumn{1}{l|}{721} &
\multicolumn{1}{l|}{750} &
\multicolumn{1}{l|}{14} \\ \hline
            \multicolumn{1}{|l|}{\multirow{2}{3cm}{SE-15 \cite{15-dataset}}} &
              %2015 &
              CitySearch New York \cite{Ganu-CitySearch} & 
              \href{https://alt.qcri.org/semeval2015/task12/index.php?id=data-and-tools}{Restaurants} &
            %   350 - 2000 
            English &
\multicolumn{1}{|l|}{350} &
\multicolumn{1}{l|}{2000} &
\multicolumn{1}{l|}{1326} &
\multicolumn{1}{l|}{496} &
\multicolumn{1}{l|}{73} &
\multicolumn{1}{l|}{1652} &
\multicolumn{1}{l|}{749} &
\multicolumn{1}{l|}{98} \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % \cite{15-dataset} &
              %2015 &
              Amazon.com &
              \href{https://alt.qcri.org/semeval2015/task12/index.php?id=data-and-tools}{Laptops} &
            %   450 - 2500 
            English &
\multicolumn{1}{|l|}{450} &
\multicolumn{1}{l|}{2500} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{1644} &
\multicolumn{1}{l|}{1094} &
\multicolumn{1}{l|}{185} \\ \hline
            \multicolumn{1}{|l|}{\multirow{11}{2.5cm}{SE-16 \cite{16-dataset}}} &
              %2016 &
              CitySearch New York \cite{Ganu-CitySearch} & 
              \href{https://alt.qcri.org/semeval2016/task5/index.php?id=data-and-tools}{Restaurants} &
            %   400 - 2286 
            English &
\multicolumn{1}{|l|}{400} &
\multicolumn{1}{l|}{2286} &
\multicolumn{1}{l|}{1817} &
\multicolumn{1}{l|}{634} &
\multicolumn{1}{l|}{106} &
\multicolumn{1}{l|}{2268} &
\multicolumn{1}{l|}{953} &
\multicolumn{1}{l|}{145} \\ \cline{2-12}
            \multicolumn{1}{|l|}{} & % \multicolumn{1}{|l|}{} & % \cite{16-dataset} &
              %2016 &
              Amazon.com &
              \href{https://alt.qcri.org/semeval2016/task5/index.php?id=data-and-tools}{Laptops} &
            %   530 - 3308 
            English &
\multicolumn{1}{|l|}{530} &
\multicolumn{1}{l|}{3308} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{2118} &
\multicolumn{1}{l|}{1358} &
\multicolumn{1}{l|}{236} \\ \cline{2-12}
              \multicolumn{1}{|l|}{} &
              %2016 &
              - & 
              \href{https://alt.qcri.org/semeval2016/task5/index.php?id=data-and-tools}{Restaurants} &
              Spanish &
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{2691} &
\multicolumn{1}{l|}{1907} &
\multicolumn{1}{l|}{672} &
\multicolumn{1}{l|}{125} &
\multicolumn{1}{l|}{2675} &
\multicolumn{1}{l|}{948} &
\multicolumn{1}{l|}{168} \\ \cline{2-12}
              \multicolumn{1}{|l|}{} &
              %2016 &
              - & 
              \href{https://alt.qcri.org/semeval2016/task5/index.php?id=data-and-tools}{Restaurants} &
              Turkish &
\multicolumn{1}{|l|}{339} &
\multicolumn{1}{l|}{1248} &
\multicolumn{1}{l|}{865} &
\multicolumn{1}{l|}{555} &
\multicolumn{1}{l|}{119} &
\multicolumn{1}{l|}{924} &
\multicolumn{1}{l|}{635} &
\multicolumn{1}{l|}{135} \\ \cline{2-12}
              \multicolumn{1}{|l|}{} &
              %2016 &
              - & 
              \href{https://alt.qcri.org/semeval2016/task5/index.php?id=data-and-tools}{Telecom} &
              Turkish &
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{3000} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} \\ \cline{2-12}
              \multicolumn{1}{|l|}{} &
              %2016 &
              - & 
              \href{https://alt.qcri.org/semeval2016/task5/index.php?id=data-and-tools}{Hotels} &
              Arabic &
\multicolumn{1}{|l|}{2291} &
\multicolumn{1}{l|}{6029} &
\multicolumn{1}{l|}{7213} &
\multicolumn{1}{l|}{4003} &
\multicolumn{1}{l|}{824} &
\multicolumn{1}{l|}{7705} &
\multicolumn{1}{l|}{4556} &
\multicolumn{1}{l|}{852} \\ \cline{2-12}
              \multicolumn{1}{|l|}{} &
              %2016 &
              - & 
              \href{https://alt.qcri.org/semeval2016/task5/index.php?id=data-and-tools}{Restaurants} &
              Dutch &
\multicolumn{1}{|l|}{400} &
\multicolumn{1}{l|}{2286} &
\multicolumn{1}{l|}{1016} &
\multicolumn{1}{l|}{546} &
\multicolumn{1}{l|}{145} &
\multicolumn{1}{l|}{1431} &
\multicolumn{1}{l|}{857} &
\multicolumn{1}{l|}{185} \\ \cline{2-12}
              \multicolumn{1}{|l|}{} &
              %2016 &
              - & 
              \href{https://alt.qcri.org/semeval2016/task5/index.php?id=data-and-tools}{Mobile Phones} &
              Dutch &
\multicolumn{1}{|l|}{270} &
\multicolumn{1}{l|}{1697} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{1454} &
\multicolumn{1}{l|}{225} &
\multicolumn{1}{l|}{110} \\ \cline{2-12}
              \multicolumn{1}{|l|}{} &
              %2016 &
              SentiRuEval-2015 \cite{SentiRuEval-2015} & 
              \href{https://alt.qcri.org/semeval2016/task5/index.php?id=data-and-tools}{Restaurants} &
              Russian &
\multicolumn{1}{|l|}{405} &
\multicolumn{1}{l|}{4699} &
\multicolumn{1}{l|}{3139} &
\multicolumn{1}{l|}{696} &
\multicolumn{1}{l|}{313} &
\multicolumn{1}{l|}{3973} &
\multicolumn{1}{l|}{1030} &
\multicolumn{1}{l|}{379} \\ \cline{2-12}
              \multicolumn{1}{|l|}{} &
              %2016 &
              - & 
              \href{https://alt.qcri.org/semeval2016/task5/index.php?id=data-and-tools}{Restaurants} &
              French &
\multicolumn{1}{|l|}{455} &
\multicolumn{1}{l|}{2429} &
\multicolumn{1}{l|}{1285} &
\multicolumn{1}{l|}{1061} &
\multicolumn{1}{l|}{289} &
\multicolumn{1}{l|}{1605} &
\multicolumn{1}{l|}{1646} &
\multicolumn{1}{l|}{233} \\ \cline{2-12}
              \multicolumn{1}{|l|}{} &
              %2016 &
              - & 
              \href{https://alt.qcri.org/semeval2016/task5/index.php?id=data-and-tools}{Mobile Phones} &
              Chinese &
\multicolumn{1}{|l|}{200} &
\multicolumn{1}{l|}{9500} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{1168} &
\multicolumn{1}{l|}{794} &
\multicolumn{1}{l|}{-} \\ \cline{2-12}
              \multicolumn{1}{|l|}{} &
              %2016 &
              - & 
              \href{https://alt.qcri.org/semeval2016/task5/index.php?id=data-and-tools}{Digital Cameras} &
              Chinese &
\multicolumn{1}{|l|}{200} &
\multicolumn{1}{l|}{8100} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{1153} &
\multicolumn{1}{l|}{587} &
\multicolumn{1}{l|}{-} \\ \hline
            SentiHood \cite{sentihood-dataset} &
              %2016 &
              Yahoo Question Answering &
              \href{https://github.com/uclnlp/jack/tree/master/data/sentihood}{Urban Neighborhoods} &
            %   N - 5215 
            English &
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{5215} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{4305} &
\multicolumn{1}{l|}{1606} &
\multicolumn{1}{l|}{-} \\ \hline
            \multicolumn{1}{|l|}{\multirow{2}{2.5cm}{Customer Response \cite{BeerAdvocate-TripAdvisor-dataset}}} &
              %2017 &
              \multicolumn{1}{|l|}{\multirow{1}{2.5cm}{www.beeradvocate .com}} & 
              \href{https://github.com/HKUST-KnowComp/DMSC}{Beer Advocate**} &
            %   {51020} 
            English &
\multicolumn{1}{|l|}{51020} &
\multicolumn{1}{l|}{552K} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{176K} &
\multicolumn{1}{l|}{8902} &
\multicolumn{1}{l|}{64K} \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % \cite{BeerAdvocate-TripAdvisor-dataset} &
              %2017 &
              \multicolumn{1}{|l|}{\multirow{1}{2.5cm}{www.tripadvisor.com}} & 
              \href{https://github.com/HKUST-KnowComp/DMSC}{Hotels**} &
            %   {29391} 
            English &
\multicolumn{1}{|l|}{29391} &
\multicolumn{1}{l|}{375K} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{120012} &
\multicolumn{1}{l|}{66017} &
\multicolumn{1}{l|}{49115} \\ \hline
            FiQA \cite{FiQA-dataset} &
              %2018 &
              Financial microblogs and headlines & 
              \href{https://sites.google.com/view/fiqa/home}{Financial**} &
            %   \begin{tabular}[c]{@{}c@{}}529 headlines \\ 774 microblogs\end{tabular} 
            English &
\multicolumn{1}{|l|}{1303} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{774} &
\multicolumn{1}{l|}{399} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{774} &
\multicolumn{1}{l|}{399} &
\multicolumn{1}{l|}{-} \\ \hline
            \multicolumn{1}{|l|}{\multirow{2}{3cm}{\cite{Bangla}}} &
              %2018 &
             FB pages, BBC Bangla, Daily Pronthom Alo &
              \href{https://github.com/AtikRahman/Bangla_ABSA_Datasets}{Cricket} &
              Bangla &
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{2691} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{571} &
\multicolumn{1}{l|}{2157} &
\multicolumn{1}{l|}{266} \\ \cline{2-12}
            \multicolumn{1}{|c|}{} & % \cite{Bangla} &
              %2018 &
             SE-14 Rest \cite{14-dataset} & 
              \href{https://github.com/AtikRahman/Bangla_ABSA_Datasets}{Restaurants} &
              Bangla &
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{1712} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{477} &
\multicolumn{1}{l|}{1226} &
\multicolumn{1}{l|}{371} \\ \hline
            \multicolumn{1}{|l|}{\multirow{2}{2.5cm}{MAMS \cite{MAMS-dataset}}} &
              %2019 &
              \multicolumn{1}{|l|}{\multirow{2}{3.5cm}{CitySearch New york \cite{Ganu-CitySearch}}} & 
              \multicolumn{1}{|l|}{\multirow{2}{2.5cm}{\href{https://github.com/siat-nlp/MAMS-for-ABSA/tree/master/data}{Restaurants}}} &
            %   N - 3849 
            English &
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{3849} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{2415} &
\multicolumn{1}{l|}{2606} &
\multicolumn{1}{l|}{3858} \\ \hline
            \multicolumn{1}{|l|}{\multirow{4}{2.5cm}{\cite{telugu-dataset}}} &
              %2020 &
              \href{123telugu.com}{123telugu}, \href{eenadu.net}{eenadu}, \href{telugu.samayam.com}{samayam} &
              \href{http://tiny.cc/vdxugz}{Movies} &
              Telugu &
\multicolumn{1}{|l|}{-} &
\multicolumn{1}{l|}{5027} &
\multicolumn{1}{l|}{2480} &
\multicolumn{1}{l|}{3251} &
\multicolumn{1}{l|}{1129} &
\multicolumn{1}{l|}{2480} &
\multicolumn{1}{l|}{3251} &
\multicolumn{1}{l|}{1129} \\ \hline
              \multicolumn{1}{|l|}{\multirow{1}{2.5cm}{ASAP \cite{chinese-rest-asap-2021}}} &
              %2018 &
              O2O e-commerce platforms &
              \href{https://github.com/Meituan-Dianping/asap/tree/master/data}{Restaurants} &
              Chinese &
\multicolumn{1}{|l|}{46700} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{-} &
\multicolumn{1}{l|}{169K} &
\multicolumn{1}{l|}{35K} &
\multicolumn{1}{l|}{66K} \\ \hline
            \end{tabular}%
        }
        \caption{Publicly available English datasets for ABSA and its subtasks. Lang.: Language, \#R: Number of Reviews, \#S: Number of Sentences. 
        **: indicates that the dataset has ratings converted to categorical sentiment polarities. Note: The domain column has a downloadable link to each dataset.  
        $\pm\pm$: indicates that those datasets have the opinion phrase annotation along with other elements.
        }
        \label{tab: Eng-Datasets}
        \end{table*}

